A Global div-curl-Lemma for Mixed Boundary Conditions in Weak Lipschitz Domains

We prove a global version of the so-called div-curl-lemma, a crucial result for compensated compactness and in homogenization theory, for mixed tangential and normal boundary conditions in bounded weak Lipschitz domains in 3D and weak Lipschitz interfaces. The crucial tools and the core of our arguments are the de Rham complex and Weck's selection theorem, the essential compact embedding result for Maxwell's equations.

==> header-pauly.tex <==

%%%%%%%%%%%%%%%%%%%%%
% LaTeX header file %
% Dirk Pauly        %
%%%%%%%%%%%%%%%%%%%%%

\usepackage[mathscr]{eucal}
\usepackage[english]{babel}
\usepackage{a4,exscale,ifthen,amsfonts,amssymb,amsmath,amscd,graphicx,color}
\usepackage{nicefrac,tikz,fancyhdr,caption,array,multirow,multicol,booktabs,algorithm,algorithmic}
\usepackage[all]{xy}

% if then
\ifthenelse{\equal{\mylabelonoff}{on}}
{\newcommand{\mylabel}[1]{\label{#1}\fbox{{\sf #1}}}}
{\newcommand{\mylabel}[1]{\label{#1}}}
%{\newcommand{\mylabel}[1]{\label{#1}\makebox[0mm][]{}}}
\ifthenelse{\equal{\allowdisbrkyesno}{yes}}
{\allowdisplaybreaks}
{}

% page outfit
\ifthenelse{\equal{\pagesizeextendednormal}{extended}}
{\setlength{\textwidth}{16cm}
\setlength{\textheight}{22cm}
\setlength{\oddsidemargin}{-0.2cm}
\setlength{\evensidemargin}{-0.2cm}}
{}
\ifthenelse{\equal{\numberingequationsectionyesno}{yes}}
{\numberwithin{equation}{section}}
{}

% colors
\newcommand{\cblack}{\color{black}}
\newcommand{\cred}{\color{red}}
\newcommand{\cpink}{\color{pink}}
\newcommand{\cmagenta}{\color{magenta}}
\newcommand{\cblue}{\color{blue}}
\newcommand{\cgreen}{\color{green}}

% this and that
\newcommand{\diss}{\displaystyle}
\newcommand{\ti}[1]{\tilde{#1}}
\newcommand{\chk}[1]{\check{#1}}
\newcommand{\ovl}[1]{\overline{#1}}
\newcommand{\unl}[1]{\underline{#1}}
\newcommand{\ovb}[1]{\overbrace{#1}}
\newcommand{\unb}[1]{\underbrace{#1}}
\newcommand{\qtext}[1]{\quad\text{#1}\quad}
\newcommand{\qqtext}[1]{\qquad\text{#1}\qquad}
\newcommand{\X}{\mathsf{X}}
\newcommand{\Y}{\mathsf{Y}}
\DeclareMathOperator{\diam}{diam}

% constants
\newcommand{\cN}{c_{N}}
\newcommand{\ctwo}{c_{2}}
\newcommand{\cNt}{\tilde{c}_{N}}
\newcommand{\cNtt}{\tilde{\tilde{c}}_{N}}

\newcommand{\cp}{c_{\mathsf{p}}}
\newcommand{\tcp}{\tilde{c}_{\mathsf{p}}}
\newcommand{\cf}{c_{\mathsf{f}}}
\newcommand{\cpf}{c_{\mathsf{p,f}}}
\newcommand{\cfp}{c_{\mathsf{f,p}}}
\newcommand{\tcf}{\tilde{c}_{\mathsf{f}}}
\newcommand{\cpN}{c_{\mathsf{p},N}}
\newcommand{\cptwo}{c_{\mathsf{p},2}}
\newcommand{\cpthree}{c_{\mathsf{p},3}}
\newcommand{\cpNrN}{c_{\mathsf{p},N,\rN}}
\newcommand{\cpNom}{c_{\mathsf{p},N,\om}}
\newcommand{\cptwortwo}{c_{\mathsf{p},2,\rtwo}}

\newcommand{\ck}{c_{\mathsf{k}}}

\newcommand{\cm}{c_{\mathsf{m}}}
\newcommand{\tcm}{\tilde{c}_{\mathsf{m}}}
\newcommand{\cmt}{c_{\mathsf{m,t}}}
\newcommand{\cmn}{c_{\mathsf{m,n}}}
\newcommand{\cmtn}{c_{\mathsf{m,t,n}}}
\newcommand{\cmnt}{c_{\mathsf{m,n,t}}}
\newcommand{\cmN}{c_{\mathsf{m},N}}
\newcommand{\cmtN}{c_{\mathsf{m,t},N}}
\newcommand{\cmtNom}{c_{\mathsf{m,t},N,\om}}
\newcommand{\cmnN}{c_{\mathsf{m,n},N}}
\newcommand{\cmnNom}{c_{\mathsf{m,n},N,\om}}
\newcommand{\cmntwoom}{c_{\mathsf{m,n},2,\om}}
\newcommand{\cmnNrN}{c_{\mathsf{m,n},N,\rN}}

\newcommand{\cstom}{c_{\om}}
\newcommand{\csthom}{\hat{c}_{\om}}
\newcommand{\csttom}{\tilde{c}_{\om}}
\newcommand{\cstoms}{c_{\oms}}

\newcommand{\ca}{c_{\A}}
\newcommand{\caa}{c_{\Aa}}

% sets
\newcommand{\set}[2]{\{#1\,:\,#2\}}
\newcommand{\setb}[2]{\big\{#1\,:\,#2\big\}}
\newcommand{\setlr}[2]{\left\{#1\,:\,#2\right\}}

% environments
\ifthenelse{\equal{\numberingtheoremsectionyesno}{yes}}
{\newtheorem{lem}{Lemma}[section]}
{\newtheorem{lem}{Lemma}}
\newtheorem{defi}[lem]{Definition}
\newtheorem{theo}[lem]{Theorem}
\newtheorem{cor}[lem]{Corollary}
\newtheorem{rem}[lem]{Remark}
\newtheorem{pro}[lem]{Proposition}
\newtheorem{ass}{Assumption}
\newtheorem{asscount}[lem]{Assumption}
\newtheorem{genass}[lem]{General Assumption}
\newtheorem{ex}[lem]{Example}
\newtheorem{algo}[lem]{Algorithm}
\newenvironment{acknow}{{\vspace*{1cm}\noindent\sc Acknowledgements }}{}

% greek letters
\newcommand{\om}{\Omega}
\newcommand{\omb}{\ovl{\om}}
\newcommand{\ombd}{\om_{\mathsf{b}}}

\newcommand{\ga}{\Gamma}
\newcommand{\gat}{\ga_{\mathsf{t}}}
\newcommand{\gan}{\ga_{\mathsf{n}}}
\newcommand{\gaD}{\ga_{\mathsf{D}}}
\newcommand{\gaN}{\ga_{\mathsf{N}}}
\newcommand{\oms}{\omega}
\newcommand{\gas}{\gamma}
\newcommand{\gaDs}{\gas_{\mathsf{D}}}
\newcommand{\gaNs}{\gas_{\mathsf{N}}}
\newcommand{\eps}{\epsilon}

% caligraphical letters
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calF}{\mathcal{F}}

% numbers and related stuff
\newcommand{\reals}{\mathbb{R}}
\newcommand{\n}{\mathbb{N}}
\newcommand{\nz}{\n_{0}}
\newcommand{\z}{\mathbb{Z}}
\newcommand{\rtwo}{\reals^{2}}
\newcommand{\rt}{\reals^{3}}
\newcommand{\rN}{\reals^{N}}
\newcommand{\rn}{\reals^{n}}
\newcommand{\rNtN}{\reals^{N\times N}}
\newcommand{\rntn}{\reals^{n\times n}}
\newcommand{\rttt}{\reals^{3\times3}}
\newcommand{\rtwottwo}{\reals^{2\times2}}

\newcommand{\foh}{\frac{1}{2}}
\newcommand{\oh}{\nicefrac{1}{2}}
\newcommand{\moh}{-\oh}
\newcommand{\fmoh}{-\foh}

% arrows
\newcommand{\ot}{\leftarrow}
\newcommand{\hookto}{\hookrightarrow}
\newcommand{\impl}{\Rightarrow}
\newcommand{\lpmi}{\Leftarrow}
\newcommand{\qimpl}{\quad\impl\quad}
\newcommand{\qqimpl}{\qquad\impl\qquad}
\newcommand{\equi}{\Leftrightarrow}
\newcommand{\qequi}{\quad\equi\quad}
\newcommand{\qqequi}{\qquad\equi\qquad}

% mappings
\newcommand{\Map}[5]{\begin{array}{ccccc}#1&:&#2&\longrightarrow&#3\\{}&{}&#4&\longmapsto&#5\end{array}}

% operators
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\sym}{sym}
\DeclareMathOperator{\skw}{skw}
\DeclareMathOperator{\dst}{dst}
\DeclareMathOperator{\dev}{dev}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\A}{A}
\DeclareMathOperator{\Almt}{\A_{\ell-2}}
\DeclareMathOperator{\Almo}{\A_{\ell-1}}
\DeclareMathOperator{\Al}{\A_{\ell}}
\DeclareMathOperator{\Alpo}{\A_{\ell+1}}
\DeclareMathOperator{\Alpt}{\A_{\ell+2}}
\DeclareMathOperator{\Aa}{\A^{\prime}}
\DeclareMathOperator{\Ap}{\A^{\prime}}
\DeclareMathOperator{\Aplmt}{\A_{\ell-2}^{\prime}}
\DeclareMathOperator{\Aplmo}{\A_{\ell-1}^{\prime}}
\DeclareMathOperator{\Apl}{\A_{\ell}^{\prime}}
\DeclareMathOperator{\Aplpo}{\A_{\ell+1}^{\prime}}
\DeclareMathOperator{\Aplpt}{\A_{\ell+2}^{\prime}}
\DeclareMathOperator{\As}{\A^{*}}
\DeclareMathOperator{\Aslmt}{\A_{\ell-2}^{*}}
\DeclareMathOperator{\Aslmo}{\A_{\ell-1}^{*}}
\DeclareMathOperator{\Asl}{\A_{\ell}^{*}}
\DeclareMathOperator{\Aslpo}{\A_{\ell+1}^{*}}
\DeclareMathOperator{\Aslpt}{\A_{\ell+2}^{*}}
\DeclareMathOperator{\cA}{\mathcal{A}}
\DeclareMathOperator{\cAlmt}{\cA_{\ell-2}}
\DeclareMathOperator{\cAlmo}{\cA_{\ell-1}}
\DeclareMathOperator{\cAl}{\cA_{\ell}}
\DeclareMathOperator{\cAlpo}{\cA_{\ell+1}}
\DeclareMathOperator{\cAlpt}{\cA_{\ell+2}}
\DeclareMathOperator{\cAa}{\cA^{\prime}}
\DeclareMathOperator{\cAp}{\cA^{\prime}}
\DeclareMathOperator{\cAplmt}{\cA_{\ell-2}^{\prime}}
\DeclareMathOperator{\cAplmo}{\cA_{\ell-1}^{\prime}}
\DeclareMathOperator{\cApl}{\cA_{\ell}^{\prime}}
\DeclareMathOperator{\cAplpo}{\cA_{\ell+1}^{\prime}}
\DeclareMathOperator{\cAplpt}{\cA_{\ell+2}^{\prime}}
\DeclareMathOperator{\cAs}{\cA^{*}}
\DeclareMathOperator{\cAslmt}{\cA_{\ell-2}^{*}}
\DeclareMathOperator{\cAslmo}{\cA_{\ell-1}^{*}}
\DeclareMathOperator{\cAsl}{\cA_{\ell}^{*}}
\DeclareMathOperator{\cAslpo}{\cA_{\ell+1}^{*}}
\DeclareMathOperator{\cAslpt}{\cA_{\ell+2}^{*}}
\DeclareMathOperator{\B}{B}
\DeclareMathOperator{\Ba}{\B^{\prime}}
\DeclareMathOperator{\cB}{\mathcal{B}}
\DeclareMathOperator{\cBa}{\cB^{\prime}}
\DeclareMathOperator{\Pot}{P}
\DeclareMathOperator{\M}{M}
\DeclareMathOperator{\cM}{\mathcal{M}}
\DeclareMathOperator{\cS}{\mathcal{S}}
\renewcommand{\S}{\mathrm{S}}
\newcommand{\tcomp}[1]{#1_{\mathsf{t}}}
\newcommand{\ncomp}[1]{#1_{\mathsf{n}}}
\DeclareMathOperator{\pilmt}{\pi_{\ell-2}}
\DeclareMathOperator{\pilmo}{\pi_{\ell-1}}
\DeclareMathOperator{\pil}{\pi_{\ell}}
\DeclareMathOperator{\pilpo}{\pi_{\ell+1}}
\DeclareMathOperator{\pilpt}{\pi_{\ell+2}}

% differential operators
\DeclareMathOperator{\p}{\partial}
\DeclareMathOperator{\na}{\nabla}
\DeclareMathOperator{\nac}{\overset{\circ}{\na}}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\rotc}{\overset{\circ}{\rot}}
\DeclareMathOperator{\rots}{rot^{*}}
\DeclareMathOperator{\Rot}{Rot}
\DeclareMathOperator{\Rotc}{\overset{\circ}{\Rot}}
\DeclareMathOperator{\Rots}{Rot^{*}}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\curls}{curl^{*}}
\DeclareMathOperator{\divergence}{div}
\renewcommand{\div}{\divergence}
\DeclareMathOperator{\divc}{\overset{\circ}{\div}}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\Divc}{\overset{\circ}{\Div}}
\DeclareMathOperator{\ed}{d}
\DeclareMathOperator{\cd}{\delta}

% C-spaces
\newcommand{\csymbol}{\mathsf{C}}
\newcommand{\cgen}[3]{\overset{#1}{\csymbol}{}^{#2}_{#3}}

\newcommand{\ci}{\cgen{}{\infty}{}}
\newcommand{\cic}{\cgen{\circ}{\infty}{}}
\newcommand{\cicgat}{\cgen{\circ}{\infty}{\gat}}
\newcommand{\cicgan}{\cgen{\circ}{\infty}{\gan}}
\newcommand{\cict}{\cgen{\circ}{\infty}{\mathsf{t}}}
\newcommand{\cicn}{\cgen{\circ}{\infty}{\mathsf{n}}}
\newcommand{\cictn}{\cgen{\circ}{\infty}{\mathsf{t,n}}}
\newcommand{\cz}{\cgen{}{0}{}}
\newcommand{\czc}{\cgen{\circ}{0}{}}
\newcommand{\czo}{\cgen{}{0,1}{}}
\newcommand{\czoc}{\cgen{\circ}{0,1}{}}
\newcommand{\co}{\cgen{}{1}{}}
\newcommand{\coc}{\cgen{\circ}{1}{}}
\newcommand{\coo}{\cgen{}{1,1}{}}
\newcommand{\cooc}{\cgen{\circ}{1,1}{}}
\newcommand{\ct}{\cgen{}{2}{}}
\newcommand{\ctc}{\cgen{\circ}{2}{}}

\renewcommand{\cir}{\ci(\reals)}
\newcommand{\cirN}{\ci(\rN)}
\newcommand{\cicrN}{\cic(\rN)}

\newcommand{\ciom}{\ci(\om)}
\newcommand{\cicom}{\cic(\om)}
\newcommand{\cicgatom}{\cicgat(\om)}
\newcommand{\cicganom}{\cicgan(\om)}
\newcommand{\cictom}{\cict(\om)}
\newcommand{\cicnom}{\cicn(\om)}
\newcommand{\cictnom}{\cictn(\om)}

\newcommand{\ciomb}{\ci(\omb)}
\newcommand{\cicomb}{\cic(\omb)}

\newcommand{\cigaom}{\cgen{}{\infty}{\ga}(\om)}
\newcommand{\cigadom}{\cgen{}{\infty}{\gaD}(\om)}
\newcommand{\cigadsoms}{\cgen{}{\infty}{\gaDs}(\oms)}

% L-spaces
\newcommand{\lsymbol}{\mathsf{L}}
\newcommand{\lgen}[3]{\overset{#1}{\lsymbol}{}^{#2}_{#3}}

\newcommand{\lt}{\lgen{}{2}{}}
\newcommand{\lo}{\lgen{}{1}{}}
\newcommand{\li}{\lgen{}{\infty}{}}

\newcommand{\lto}{\lgen{}{2}{1}}
\newcommand{\ltmo}{\lgen{}{2}{-1}}
\newcommand{\ltz}{\lgen{}{2}{0}}
\newcommand{\lts}{\lgen{}{2}{s}}
\newcommand{\ltt}{\lgen{}{2}{t}}
\newcommand{\ltsmo}{\lgen{}{2}{s-1}}
\newcommand{\ltspo}{\lgen{}{2}{s+1}}

\newcommand{\ltloc}{\lgen{}{2}{\mathsf{loc}}}
\newcommand{\ltvox}{\lgen{}{2}{\mathsf{vox}}}
\newcommand{\ltbot}{\lgen{}{2}{\bot}}
\newcommand{\lteps}{\lgen{}{2}{\eps}}
\newcommand{\ltmu}{\lgen{}{2}{\mu}}

\newcommand{\ltga}{\lgen{}{2}{\ga}}
\newcommand{\ltgas}{\lgen{}{2}{\gas}}
\newcommand{\ltgad}{\lgen{}{2}{\gaD}}
\newcommand{\ltgads}{\lgen{}{2}{\gaDs}}

\newcommand{\lir}{\li(\reals)}
\newcommand{\ltrN}{\lt(\rN)}
\newcommand{\ltrtwo}{\lt(\rtwo)}
\newcommand{\ltrt}{\lt(\rt)}
\newcommand{\ltom}{\lt(\om)}
\newcommand{\loom}{\lo(\om)}
\newcommand{\liom}{\li(\om)}
\newcommand{\ltoms}{\lt(\oms)}

\newcommand{\ltmorN}{\ltmo(\rN)}
\newcommand{\ltmoom}{\ltmo(\om)}
\newcommand{\ltsom}{\lts(\om)}
\newcommand{\ltsmoom}{\ltsmo(\om)}
\newcommand{\ltspoom}{\ltspo(\om)}
\newcommand{\lttom}{\ltt(\om)}
\newcommand{\ltzom}{\ltz(\om)}

\newcommand{\ltlocrN}{\ltloc(\rN)}
\newcommand{\ltlocom}{\ltloc(\om)}
\newcommand{\ltvoxrN}{\ltvox(\rN)}
\newcommand{\ltvoxom}{\ltvox(\om)}
\newcommand{\ltlocomb}{\ltloc(\omb)}
\newcommand{\ltbotom}{\ltbot(\om)}
\newcommand{\ltepsom}{\lteps(\om)}
\newcommand{\ltmuom}{\ltmu(\om)}

\newcommand{\ltgadom}{\ltgad(\om)}
\newcommand{\ltvoxgadom}{\lgen{}{2}{\mathsf{vox},\gaD}(\om)}
\newcommand{\ltgasoms}{\ltgas(\oms)}
\newcommand{\ltgadsoms}{\ltgads(\oms)}

% L-tilde-spaces
\newcommand{\ltilde}[3]{\overset{#1}{\tilde{\lsymbol}}{}^{#2}_{#3}}

\newcommand{\ltildet}{\ltilde{}{2}{}}
\newcommand{\ltildets}{\ltilde{}{2}{s}}
\newcommand{\ltildetmo}{\ltilde{}{2}{-1}}

\newcommand{\ltildetsrN}{\ltildets(\rN)}
\newcommand{\ltildetsom}{\ltildets(\om)}
\newcommand{\ltildetmorN}{\ltildetmo(\rN)}
\newcommand{\ltildetmoom}{\ltildetmo(\om)}

% H-spaces
\newcommand{\hsymbol}{\mathsf{H}}
\newcommand{\Hsymbol}{\text{\sf\bfseries H}}
\newcommand{\hgen}[3]{\overset{#1}{\hsymbol}{}^{#2}_{#3}}
\newcommand{\Hgen}[3]{\overset{#1}{\Hsymbol}{}^{#2}_{#3}}

\newcommand{\hz}{\hgen{}{0}{}}
\newcommand{\ho}{\hgen{}{1}{}}
\newcommand{\htwo}{\hgen{}{2}{}}
\newcommand{\hl}{\hgen{}{\ell}{}}
\newcommand{\hlpo}{\hgen{}{\ell+1}{}}
\newcommand{\hlpt}{\hgen{}{\ell+2}{}}
\newcommand{\Ho}{\Hgen{}{1}{}}
\newcommand{\hoc}{\hgen{\circ}{1}{}}
\newcommand{\htwoc}{\hgen{\circ}{2}{}}
\newcommand{\hocga}{\hgen{\circ}{1}{\ga}}
\newcommand{\hocgat}{\hgen{\circ}{1}{\gat}}
\newcommand{\hocgan}{\hgen{\circ}{1}{\gan}}
\newcommand{\hlc}{\hgen{\circ}{\ell}{}}
\newcommand{\hlcga}{\hgen{\circ}{\ell}{\ga}}
\newcommand{\hlcgat}{\hgen{\circ}{\ell}{\gat}}
\newcommand{\hlcgan}{\hgen{\circ}{\ell}{\gan}}
\newcommand{\hlpoc}{\hgen{\circ}{\ell+1}{}}
\newcommand{\hlptc}{\hgen{\circ}{\ell+2}{}}
\newcommand{\hobot}{\hgen{}{1}{\bot}}
\newcommand{\hlbot}{\hgen{}{\ell}{\bot}}
\newcommand{\hocbot}{\hgen{\circ}{1}{\bot}}
\newcommand{\hlcbot}{\hgen{\circ}{\ell}{\bot}}
\newcommand{\hoct}{\hgen{\circ}{1}{\mathsf{t}}}
\newcommand{\hocn}{\hgen{\circ}{1}{\mathsf{n}}}
\newcommand{\hoctn}{\hgen{\circ}{1}{\mathsf{t,n}}}

\newcommand{\hoz}{\hgen{}{1}{0}}
\newcommand{\hos}{\hgen{}{1}{s}}
\newcommand{\hosmo}{\hgen{}{1}{s-1}}
\newcommand{\hospo}{\hgen{}{1}{s+1}}
\newcommand{\Hoz}{\Hgen{}{1}{0}}
\newcommand{\Hos}{\Hgen{}{1}{s}}
\newcommand{\Hosmo}{\Hgen{}{1}{s-1}}
\newcommand{\Hospo}{\Hgen{}{1}{s+1}}
\newcommand{\hot}{\hgen{}{1}{t}}
\newcommand{\Hot}{\Hgen{}{1}{t}}
\newcommand{\homo}{\hgen{}{1}{-1}}
\newcommand{\hosc}{\hgen{\circ}{1}{s}}
\newcommand{\hotc}{\hgen{\circ}{1}{t}}
\newcommand{\homoc}{\hgen{\circ}{1}{-1}}

\newcommand{\hocgatn}{\hgen{\circ}{1}{\ga_{\mathsf{t}},\ga_{\mathsf{n}}}}
\newcommand{\hoga}{\hgen{}{1}{\ga}}
\newcommand{\Hoga}{\Hgen{}{1}{\ga}}
\newcommand{\hogas}{\hgen{}{1}{\gas}}
\newcommand{\hogad}{\hgen{}{1}{\gaD}}
\newcommand{\Hogad}{\Hgen{}{1}{\gaD}}
\newcommand{\hogan}{\hgen{}{1}{\gaN}}
\newcommand{\hogads}{\hgen{}{1}{\gaDs}}

\newcommand{\homoctn}{\hgen{\circ}{1}{-1,\mathsf{t,n}}}
\newcommand{\hosga}{\hgen{}{1}{s,\ga}}
\newcommand{\homoga}{\hgen{}{1}{-1,\ga}}
\newcommand{\hosgad}{\hgen{}{1}{s,\gaD}}
\newcommand{\Hozgad}{\Hgen{}{1}{0,\gaD}}
\newcommand{\Hosgad}{\Hgen{}{1}{s,\gaD}}
\newcommand{\homogad}{\hgen{}{1}{-1,\gaD}}
\newcommand{\hosgan}{\hgen{}{1}{s,\gaN}}
\newcommand{\homogan}{\hgen{}{1}{-1,\gaN}}

\newcommand{\horN}{\ho(\rN)}
\newcommand{\hzom}{\hz(\om)}
\newcommand{\hoom}{\ho(\om)}
\newcommand{\hooms}{\ho(\oms)}
\newcommand{\htom}{\htwo(\om)}
\newcommand{\hlom}{\hl(\om)}
\newcommand{\hlpoom}{\hlpo(\om)}
\newcommand{\hlptom}{\hlpt(\om)}
\newcommand{\HorN}{\Ho(\rN)}
\newcommand{\Hoom}{\Ho(\om)}
\newcommand{\hocom}{\hoc(\om)}
\newcommand{\hocgaom}{\hocga(\om)}
\newcommand{\hocgatom}{\hocgat(\om)}
\newcommand{\hocganom}{\hocgan(\om)}
\newcommand{\htcom}{\htwoc(\om)}
\newcommand{\hlcom}{\hlc(\om)}
\newcommand{\hlcgaom}{\hlcga(\om)}
\newcommand{\hlcgatom}{\hlcgat(\om)}
\newcommand{\hlcganom}{\hlcgan(\om)}
\newcommand{\hlpocom}{\hlpoc(\om)}
\newcommand{\hlptcom}{\hlptc(\om)}
\newcommand{\hobotom}{\hobot(\om)}
\newcommand{\hocbotom}{\hocbot(\om)}
\newcommand{\hlbotom}{\hlbot(\om)}
\newcommand{\hlcbotom}{\hlcbot(\om)}
\newcommand{\hoctom}{\hoct(\om)}
\newcommand{\hocnom}{\hocn(\om)}
\newcommand{\hoctnom}{\hoctn(\om)}
\newcommand{\homoctnom}{\homoctn(\om)}

\newcommand{\hogaom}{\hoga(\om)}
\newcommand{\Hogaom}{\Hoga(\om)}
\newcommand{\hogadom}{\hogad(\om)}
\newcommand{\hoganom}{\hogan(\om)}

\newcommand{\hogasoms}{\hogas(\oms)}
\newcommand{\hogadsoms}{\hogads(\oms)}

\newcommand{\hosrN}{\hos(\rN)}
\newcommand{\homorN}{\homo(\rN)}
\newcommand{\hozom}{\hoz(\om)}
\newcommand{\hosom}{\hos(\om)}
\newcommand{\hosmoom}{\hosmo(\om)}
\newcommand{\hospoom}{\hospo(\om)}
\newcommand{\Hozom}{\Hoz(\om)}
\newcommand{\Hosom}{\Hos(\om)}
\newcommand{\Hosmoom}{\Hosmo(\om)}
\newcommand{\Hospoom}{\Hospo(\om)}
\newcommand{\hotom}{\hot(\om)}
\newcommand{\Hotom}{\Hot(\om)}
\newcommand{\homoom}{\homo(\om)}
\newcommand{\hoscom}{\hosc(\om)}
\newcommand{\hotcom}{\hotc(\om)}
\newcommand{\homocom}{\homoc(\om)}

\newcommand{\hosgaom}{\hosga(\om)}
\newcommand{\homogaom}{\homoga(\om)}
\newcommand{\hosgadom}{\hosgad(\om)}
\newcommand{\Hogadom}{\Hogad(\om)}
\newcommand{\Hozgadom}{\Hozgad(\om)}
\newcommand{\Hosgadom}{\Hosgad(\om)}
\newcommand{\homogadom}{\homogad(\om)}
\newcommand{\hosganom}{\hosgan(\om)}
\newcommand{\homoganom}{\homogan(\om)}

% H-tilde-spaces
\newcommand{\htilde}[3]{\overset{#1}{\tilde{\hsymbol}}{}^{#2}_{#3}}

\newcommand{\htildeo}{\htilde{}{1}{}}
\newcommand{\htildeos}{\htilde{}{1}{s}}
\newcommand{\htildeomo}{\htilde{}{1}{-1}}

\newcommand{\htildeoga}{\htilde{}{1}{\ga}}
\newcommand{\htildeosga}{\htilde{}{1}{s,\ga}}
\newcommand{\htildeomoga}{\htilde{}{1}{-1,\ga}}
\newcommand{\htildeogad}{\htilde{}{1}{\gaD}}
\newcommand{\htildeosgad}{\htilde{}{1}{s,\gaD}}
\newcommand{\htildeomogad}{\htilde{}{1}{-1,\gaD}}

\newcommand{\htildeosrN}{\htildeos(\rN)}
\newcommand{\htildeosom}{\htildeos(\om)}
\newcommand{\htildeosgaom}{\htildeosga(\om)}
\newcommand{\htildeosgadom}{\htildeosgad(\om)}
\newcommand{\htildeomorN}{\htildeomo(\rN)}
\newcommand{\htildeomoom}{\htildeomo(\om)}
\newcommand{\htildeomogaom}{\htildeomoga(\om)}
\newcommand{\htildeomogadom}{\htildeomogad(\om)}

% dual H-spaces
\newcommand{\hmo}{\hgen{}{-1}{}}
\newcommand{\hmoom}{\hmo(\om)}
\newcommand{\hmt}{\hgen{}{-2}{}}
\newcommand{\hmtom}{\hmt(\om)}
\newcommand{\hml}{\hgen{}{-\ell}{}}
\newcommand{\hmlpo}{\hgen{}{-\ell+1}{}}
\newcommand{\hmlmo}{\hgen{}{-\ell-1}{}}
\newcommand{\hmlmt}{\hgen{}{-\ell-2}{}}
\newcommand{\hmlom}{\hml(\om)}
\newcommand{\hmlpoom}{\hmlpo(\om)}
\newcommand{\hmlmoom}{\hmlmo(\om)}
\newcommand{\hmlmtom}{\hmlmt(\om)}

% H-spaces fractional
\newcommand{\hoh}{\hgen{}{\oh}{}}
\newcommand{\hmoh}{\hgen{}{\moh}{}}
\newcommand{\hohga}{\hoh(\ga)}
\newcommand{\hmohga}{\hmoh(\ga)}

% W-spaces
\newcommand{\wsymbol}{\mathsf{W}}
\newcommand{\wgen}[3]{\overset{#1}{\wsymbol}{}^{#2}_{#3}}

\newcommand{\wo}{\wgen{}{1}{}}
\newcommand{\woi}{\wgen{}{1,\infty}{}}

\newcommand{\woirN}{\woi(\rN)}
\newcommand{\woom}{\woi(\om)}

% R-spaces
\newcommand{\rsymbol}{\mathsf{R}}
\newcommand{\Rsymbol}{\text{\sf\bfseries R}}
\newcommand{\rgen}[3]{\overset{#1}{\rsymbol}{}^{#2}_{#3}}
\newcommand{\Rgen}[3]{\overset{#1}{\Rsymbol}{}^{#2}_{#3}}

\renewcommand{\r}{\rgen{}{}{}}
\newcommand{\rhmo}{\rgen{}{-1}{}}
\newcommand{\rhml}{\rgen{}{-\ell}{}}
\newcommand{\rhmlmo}{\rgen{}{-\ell-1}{}}
\newcommand{\rhmoz}{\rgen{}{-1}{0}}
\newcommand{\rhmlz}{\rgen{}{-\ell}{0}}
\newcommand{\rhmlmoz}{\rgen{}{-\ell-1}{0}}
\newcommand{\R}{\Rgen{}{}{}}
\newcommand{\rz}{\rgen{}{}{0}}
\newcommand{\Rz}{\Rgen{}{}{0}}
\newcommand{\rc}{\rgen{\circ}{}{}}
\newcommand{\Rc}{\Rgen{\circ}{}{}}
\newcommand{\rcz}{\rgen{\circ}{}{0}}
%\newcommand{\rcgat}{\rgen{\circ}{}{\ga_{\mathsf{t}}}}
\newcommand{\rcga}{\rgen{\circ}{}{\ga}}
\newcommand{\rcgat}{\rgen{\circ}{}{\gat}}
\newcommand{\rcgan}{\rgen{\circ}{}{\gan}}
\newcommand{\rga}{\rgen{}{}{\ga}}
\newcommand{\rgat}{\rgen{}{}{\gat}}
\newcommand{\rgan}{\rgen{}{}{\gan}}
\newcommand{\Rga}{\Rgen{}{}{\ga}}
\newcommand{\rgad}{\rgen{}{}{\gaD}}
\newcommand{\Rgad}{\Rgen{}{}{\gaD}}
\newcommand{\rgaz}{\rgen{}{}{\ga,0}}
\newcommand{\rgatz}{\rgen{}{}{\gat,0}}
\newcommand{\rganz}{\rgen{}{}{\gan,0}}
\newcommand{\rcgaz}{\rgen{\circ}{}{\ga,0}}
\newcommand{\rcgatz}{\rgen{\circ}{}{\gat,0}}
\newcommand{\rcganz}{\rgen{\circ}{}{\gan,0}}
\newcommand{\Rgaz}{\Rgen{}{}{\ga,0}}
\newcommand{\rgadz}{\rgen{}{}{\gaD,0}}
\newcommand{\Rgadz}{\Rgen{}{}{\gaD,0}}

\newcommand{\rs}{\rgen{}{}{s}}
\newcommand{\rsz}{\rgen{}{}{s,0}}
\newcommand{\Rs}{\Rgen{}{}{s}}
\newcommand{\Rsz}{\Rgen{}{}{s,z}}
\newcommand{\rmo}{\rgen{}{}{-1}}
\newcommand{\rmoz}{\rgen{}{}{-1,0}}
\newcommand{\rmoga}{\rgen{}{}{-1,\ga}}
\newcommand{\rsga}{\rgen{}{}{s,\ga}}
\newcommand{\rsgaz}{\rgen{}{}{s,\ga,0}}
\newcommand{\rzgad}{\rgen{}{}{0,\gaD}}
\newcommand{\rmogad}{\rgen{}{}{-1,\gaD}}
\newcommand{\rmogadz}{\rgen{}{}{-1,\gaD,0}}
\newcommand{\rsgad}{\rgen{}{}{s,\gaD}}
\newcommand{\rsgadz}{\rgen{}{}{s,\gaD,0}}
\newcommand{\rmogaz}{\rgen{}{}{-1,\ga,0}}
\newcommand{\rsc}{\rgen{\circ}{}{s}}
\newcommand{\rscz}{\rgen{\circ}{}{s,0}}
\newcommand{\rmoc}{\rgen{\circ}{}{-1}}

\newcommand{\rrN}{\r(\rN)}
\newcommand{\rom}{\r(\om)}
\newcommand{\rcom}{\rc(\om)}
\newcommand{\rczom}{\rcz(\om)}
\newcommand{\rhmoom}{\rhmo(\om)}
\newcommand{\rhmlom}{\rhml(\om)}
\newcommand{\rhmlmoom}{\rhmlmo(\om)}
\newcommand{\rhmozom}{\rhmoz(\om)}
\newcommand{\rhmlzom}{\rhmlz(\om)}
\newcommand{\rhmlmozom}{\rhmlmoz(\om)}
\newcommand{\Rom}{\R(\om)}
\newcommand{\Rcom}{\Rc(\om)}
\newcommand{\rzom}{\rz(\om)}
\newcommand{\Rzom}{\Rz(\om)}
\newcommand{\rgaom}{\rga(\om)}
\newcommand{\Rgaom}{\Rga(\om)}
\newcommand{\rgatom}{\rgat(\om)}
\newcommand{\rganom}{\rgan(\om)}
\newcommand{\rcgaom}{\rcga(\om)}
\newcommand{\rcgatom}{\rcgat(\om)}
\newcommand{\rcganom}{\rcgan(\om)}
\newcommand{\rgatzom}{\rgatz(\om)}
\newcommand{\rganzom}{\rganz(\om)}
\newcommand{\rcgazom}{\rcgaz(\om)}
\newcommand{\rcgatzom}{\rcgatz(\om)}
\newcommand{\rcganzom}{\rcganz(\om)}
\newcommand{\rgadom}{\rgad(\om)}
\newcommand{\Rgadom}{\Rgad(\om)}
\newcommand{\rgazom}{\rgaz(\om)}
\newcommand{\Rgazom}{\Rgaz(\om)}
\newcommand{\rgadzom}{\rgadz(\om)}
\newcommand{\Rgadzom}{\Rgadz(\om)}

\newcommand{\rsom}{\rs(\om)}
\newcommand{\rszom}{\rsz(\om)}
\newcommand{\rmorN}{\rmo(\rN)}
\newcommand{\rmoom}{\rmo(\om)}
\newcommand{\rmozrN}{\rmoz(\rN)}
\newcommand{\rmozom}{\rmoz(\om)}
\newcommand{\rmogaom}{\rmoga(\om)}
\newcommand{\rmogazom}{\rmogaz(\om)}
\newcommand{\rzgadom}{\rzgad(\om)}
\newcommand{\rmogadom}{\rmogad(\om)}
\newcommand{\rmogadzom}{\rmogadz(\om)}
\newcommand{\rsgaom}{\rsga(\om)}
\newcommand{\rsgadom}{\rsgad(\om)}
\newcommand{\rsgazom}{\rsgaz(\om)}
\newcommand{\rsgadzom}{\rsgadz(\om)}

% Rstar-spaces
\newcommand{\rstargen}[2]{\overset{#1}{\rsymbol}{}^{*}_{#2}}
\newcommand{\Rstargen}[2]{\overset{#1}{\Rsymbol}{}^{*}_{#2}}

\newcommand{\rstar}{\rstargen{}{}}
\newcommand{\Rstar}{\Rstargen{}{}}
\newcommand{\rstarz}{\rstargen{}{0}}
\newcommand{\Rstarz}{\Rstargen{}{0}}
\newcommand{\rstarc}{\rstargen{\circ}{}}
\newcommand{\rstarcgat}{\rstargen{\circ}{\ga_{\mathsf{t}}}}
\newcommand{\rstarga}{\rstargen{}{\ga}}
\newcommand{\Rstarga}{\Rstargen{}{\ga}}
\newcommand{\Rstargad}{\Rstargen{}{\gaD}}
\newcommand{\rstargaz}{\rstargen{}{\ga,0}}
\newcommand{\Rstargaz}{\Rstargen{}{\ga,0}}

\newcommand{\rstars}{\rstargen{}{s}}
\newcommand{\Rstars}{\Rstargen{}{s}}
\newcommand{\rstarmo}{\rstargen{}{-1}}
\newcommand{\rstarmoz}{\rstargen{}{-1,0}}
\newcommand{\rstarmoga}{\rstargen{}{-1,\ga}}
\newcommand{\rstarsga}{\rstargen{}{s,\ga}}
\newcommand{\rstarmogad}{\rstargen{}{-1,\gaD}}
\newcommand{\rstarsgad}{\rstargen{}{s,\gaD}}
\newcommand{\rstarmogaz}{\rstargen{}{-1,\ga,0}}
\newcommand{\starrsc}{\rstargen{\circ}{s}}
\newcommand{\rstarmoc}{\rstargen{\circ}{-1}}

\newcommand{\rstarrN}{\rstar(\rN)}
\newcommand{\rstarom}{\rstar(\om)}
\newcommand{\rstarsom}{\rstars(\om)}
\newcommand{\Rstarom}{\Rstar(\om)}
\newcommand{\rstarzom}{\rstarz(\om)}
\newcommand{\Rstarzom}{\Rstarz(\om)}
\newcommand{\rstargaom}{\rstarga(\om)}
\newcommand{\Rstargaom}{\Rstarga(\om)}
\newcommand{\Rstargadom}{\Rstargad(\om)}
\newcommand{\rstargazom}{\rstargaz(\om)}
\newcommand{\Rstargazom}{\Rstargaz(\om)}

\newcommand{\rstarmorN}{\rstarmo(\rN)}
\newcommand{\rstarmoom}{\rstarmo(\om)}
\newcommand{\rstarmozom}{\rstarmoz(\om)}
\newcommand{\rstarmogaom}{\rstarmoga(\om)}
\newcommand{\rstarmogazom}{\rstarmogaz(\om)}
\newcommand{\rstarmogadom}{\rstarmogad(\om)}
\newcommand{\rstarsgadom}{\rstarsgad(\om)}

% R-tilde-spaces
\newcommand{\rtildegen}[3]{\overset{#1}{\tilde{\rsymbol}}{}^{#2}_{#3}}

\newcommand{\rtilde}{\rtildegen{}{}{}}
\newcommand{\rtildega}{\rtildegen{}{}{\ga}}
\newcommand{\rtildegad}{\rtildegen{}{}{\gaD}}

\newcommand{\rtildes}{\rtildegen{}{}{s}}
\newcommand{\rtildemo}{\rtildegen{}{}{-1}}
\newcommand{\rtildesga}{\rtildegen{}{}{s,\ga}}
\newcommand{\rtildemoga}{\rtildegen{}{}{-1,\ga}}
\newcommand{\rtildesgad}{\rtildegen{}{}{s,\gaD}}
\newcommand{\rtildemogad}{\rtildegen{}{}{-1,\gaD}}

\newcommand{\rtildesrN}{\rtildes(\rN)}
\newcommand{\rtildesom}{\rtildes(\om)}
\newcommand{\rtildesgaom}{\rtildesga(\om)}
\newcommand{\rtildesgadom}{\rtildesgad(\om)}
\newcommand{\rtildemorN}{\rtildemo(\rN)}
\newcommand{\rtildemoom}{\rtildemo(\om)}
\newcommand{\rtildemogaom}{\rtildemoga(\om)}
\newcommand{\rtildemogadom}{\rtildemogad(\om)}

% D-spaces
\newcommand{\dsymbol}{\mathsf{D}}
\newcommand{\Dsymbol}{\text{\sf\bfseries D}}
\newcommand{\dgen}[3]{\overset{#1}{\dsymbol}{}^{#2}_{#3}}
\newcommand{\Dgen}[3]{\overset{#1}{\Dsymbol}{}^{#2}_{#3}}

\renewcommand{\d}{\dgen{}{}{}}
\newcommand{\D}{\Dgen{}{}{}}
\newcommand{\dhmo}{\dgen{}{-1}{}}
\newcommand{\dhml}{\dgen{}{-\ell}{}}
\newcommand{\dhmlmo}{\dgen{}{-\ell-1}{}}
\newcommand{\dhmoz}{\dgen{}{-1}{0}}
\newcommand{\dhmlz}{\dgen{}{-\ell}{0}}
\newcommand{\dhmlmoz}{\dgen{}{-\ell-1}{0}}
\newcommand{\dz}{\dgen{}{}{0}}
\newcommand{\Dz}{\Dgen{}{}{0}}
\newcommand{\dc}{\dgen{\circ}{}{}}
\newcommand{\dcz}{\dgen{\circ}{}{0}}
%\newcommand{\dcgan}{\dgen{\circ}{}{\ga_{\mathsf{n}}}}
\newcommand{\dcga}{\dgen{\circ}{}{\ga}}
\newcommand{\dcgat}{\dgen{\circ}{}{\gat}}
\newcommand{\dcgan}{\dgen{\circ}{}{\gan}}
\newcommand{\dcgaz}{\dgen{\circ}{}{\ga,0}}
\newcommand{\dcgatz}{\dgen{\circ}{}{\gat,0}}
\newcommand{\dcganz}{\dgen{\circ}{}{\gan,0}}
\newcommand{\dga}{\dgen{}{}{\ga}}
\newcommand{\Dga}{\Dgen{}{}{\ga}}
\newcommand{\dgat}{\dgen{}{}{\gat}}
\newcommand{\dgan}{\dgen{}{}{\gan}}
\newcommand{\dgatz}{\dgen{}{}{\gat,0}}
\newcommand{\dganz}{\dgen{}{}{\gan,0}}
\newcommand{\Dgad}{\Dgen{}{}{\gaD}}
\newcommand{\dgaz}{\dgen{}{}{\ga,0}}
\newcommand{\Dgaz}{\Dgen{}{}{\ga,0}}
\newcommand{\dgasz}{\dgen{}{}{\gas,0}}
\newcommand{\dgadz}{\dgen{}{}{\gaD,0}}
\newcommand{\Dgadz}{\Dgen{}{}{\gaD,0}}

\newcommand{\ds}{\dgen{}{}{s}}
\newcommand{\dsz}{\dgen{}{}{s,0}}
\newcommand{\Ds}{\Dgen{}{}{s}}
\newcommand{\Dsz}{\Dgen{}{}{s,0}}
\newcommand{\dmo}{\dgen{}{}{-1}}
\newcommand{\dmoz}{\dgen{}{}{-1,0}}
\newcommand{\dmoga}{\dgen{}{}{-1,\ga}}
\newcommand{\dsga}{\dgen{}{}{s,\ga}}
\newcommand{\dsgaz}{\dgen{}{}{s,\ga,0}}
\newcommand{\dmogad}{\dgen{}{}{-1,\gaD}}
\newcommand{\dmogadz}{\dgen{}{}{-1,\gaD,0}}
\newcommand{\dsgad}{\dgen{}{}{s,\gaD}}
\newcommand{\dsgadz}{\dgen{}{}{s,\gaD,0}}
\newcommand{\dmogaz}{\dgen{}{}{-1,\ga,0}}
\newcommand{\dsc}{\dgen{\circ}{}{s}}
\newcommand{\dscz}{\dgen{\circ}{}{s,0}}
\newcommand{\dmoc}{\dgen{\circ}{}{-1}}
\newcommand{\dmocz}{\dgen{\circ}{}{-1,0}}

\newcommand{\drN}{\d(\rN)}
\newcommand{\dom}{\d(\om)}
\newcommand{\Dom}{\D(\om)}
\newcommand{\dcom}{\dc(\om)}
\newcommand{\dzom}{\dz(\om)}
\newcommand{\dczom}{\dcz(\om)}
\newcommand{\dhmoom}{\dhmo(\om)}
\newcommand{\dhmlom}{\dhml(\om)}
\newcommand{\dhmlmoom}{\dhmlmo(\om)}
\newcommand{\dhmozom}{\dhmoz(\om)}
\newcommand{\dhmlzom}{\dhmlz(\om)}
\newcommand{\dhmlmozom}{\dhmlmoz(\om)}
\newcommand{\Dzom}{\Dz(\om)}
\newcommand{\dgatom}{\dgat(\om)}
\newcommand{\dganom}{\dgan(\om)}
\newcommand{\dcgaom}{\dcga(\om)}
\newcommand{\dcgatom}{\dcgat(\om)}
\newcommand{\dcganom}{\dcgan(\om)}
\newcommand{\dgatzom}{\dgatz(\om)}
\newcommand{\dganzom}{\dganz(\om)}
\newcommand{\dcgazom}{\dcgaz(\om)}
\newcommand{\dcgatzom}{\dcgatz(\om)}
\newcommand{\dcganzom}{\dcganz(\om)}
\newcommand{\dgaom}{\dga(\om)}
\newcommand{\Dgaom}{\Dga(\om)}
\newcommand{\Dgadom}{\Dgad(\om)}
\newcommand{\dgazom}{\dgaz(\om)}
\newcommand{\Dgazom}{\Dgaz(\om)}
\newcommand{\dgaszoms}{\dgasz(\oms)}
\newcommand{\dgadzom}{\dgadz(\om)}
\newcommand{\Dgadzom}{\Dgadz(\om)}

\newcommand{\dmorN}{\dmo(\rN)}
\newcommand{\dsom}{\ds(\om)}
\newcommand{\dszom}{\dsz(\om)}
\newcommand{\dmoom}{\dmo(\om)}
\newcommand{\dmozom}{\dmoz(\om)}
\newcommand{\dmogaom}{\dmoga(\om)}
\newcommand{\dmogazom}{\dmogaz(\om)}
\newcommand{\dmogadom}{\dmogad(\om)}
\newcommand{\dmogadzom}{\dmogadz(\om)}
\newcommand{\dsgaom}{\dsga(\om)}
\newcommand{\dsgazom}{\dsgaz(\om)}
\newcommand{\dsgadom}{\dsgad(\om)}
\newcommand{\dsgadzom}{\dsgadz(\om)}

% D-tilde-spaces
\newcommand{\dtildegen}[3]{\overset{#1}{\tilde{\dsymbol}}{}^{#2}_{#3}}

\newcommand{\dtilde}{\dtildegen{}{}{}}
\newcommand{\dtildega}{\dtildegen{}{}{\ga}}
\newcommand{\dtildegad}{\dtildegen{}{}{\gaD}}

\newcommand{\dtildes}{\dtildegen{}{}{s}}
\newcommand{\dtildemo}{\dtildegen{}{}{-1}}
\newcommand{\dtildesga}{\dtildegen{}{}{s,\ga}}
\newcommand{\dtildemoga}{\dtildegen{}{}{-1,\ga}}
\newcommand{\dtildesgad}{\dtildegen{}{}{s,\gaD}}
\newcommand{\dtildemogad}{\dtildegen{}{}{-1,\gaD}}

\newcommand{\dtildesrN}{\dtildes(\rN)}
\newcommand{\dtildesom}{\dtildes(\om)}
\newcommand{\dtildesgaom}{\dtildesga(\om)}
\newcommand{\dtildesgadom}{\dtildesgad(\om)}
\newcommand{\dtildemorN}{\dtildemo(\rN)}
\newcommand{\dtildemoom}{\dtildemo(\om)}
\newcommand{\dtildemogaom}{\dtildemoga(\om)}
\newcommand{\dtildemogadom}{\dtildemogad(\om)}

% G-spaces
\newcommand{\gsymbol}{\mathsf{G}}
\newcommand{\ggen}[3]{\overset{#1}{\gsymbol}{}^{#2}_{#3}}

\newcommand{\ghmo}{\ggen{}{-1}{}}
\newcommand{\ghml}{\ggen{}{-\ell}{}}
\newcommand{\ghmlmo}{\ggen{}{-\ell-1}{}}
\newcommand{\ghmoz}{\ggen{}{-1}{0}}
\newcommand{\ghmlz}{\ggen{}{-\ell}{0}}
\newcommand{\ghmlmoz}{\ggen{}{-\ell-1}{0}}

\newcommand{\ghmoom}{\ghmo(\om)}
\newcommand{\ghmlom}{\ghml(\om)}
\newcommand{\ghmlmoom}{\ghmlmo(\om)}
\newcommand{\ghmozom}{\ghmoz(\om)}
\newcommand{\ghmlzom}{\ghmlz(\om)}
\newcommand{\ghmlmozom}{\ghmlmoz(\om)}

% harmonic fields
\newcommand{\harmsymbol}{\mathcal{H}}
\newcommand{\harmgen}[3]{\overset{#1}{\harmsymbol}{}^{#2}_{#3}}

\newcommand{\harm}{\harmgen{}{}{}}
\newcommand{\harmd}{\harmgen{}{}{\mathsf{D}}}
\newcommand{\harmdz}{\harmgen{}{}{\mathsf{D},0}}
\newcommand{\harmdmo}{\harmgen{}{}{\mathsf{D},-1}}
\newcommand{\harmom}{\harm(\om)}
\newcommand{\harmdom}{\harmd(\om)}
\newcommand{\harmdzom}{\harmdz(\om)}
\newcommand{\harmdmoom}{\harmdmo(\om)}

\newcommand{\harmn}{\harmgen{}{}{\mathsf{N}}}
\newcommand{\harmnz}{\harmgen{}{}{\mathsf{N},0}}
\newcommand{\harmnmo}{\harmgen{}{}{\mathsf{N},-1}}
\newcommand{\harmnom}{\harmn(\om)}
\newcommand{\harmnzom}{\harmnz(\om)}
\newcommand{\harmnmoom}{\harmnmo(\om)}

% Banach/Hilbert spaces
\newcommand{\banach}{\hsymbol}
\newcommand{\banachz}{\banach_{0}}
\newcommand{\banachzp}{\banach_{0}^{\prime}}
\newcommand{\banacho}{\banach_{1}}
\newcommand{\banachop}{\banach_{1}^{\prime}}
\newcommand{\banacht}{\banach_{2}}
\newcommand{\banachtp}{\banach_{2}^{\prime}}
\newcommand{\hilbert}{\hsymbol}
\newcommand{\hilz}{\hilbert_{0}}
\newcommand{\hilo}{\hilbert_{1}}
\newcommand{\hilt}{\hilbert_{2}}
\newcommand{\hilthr}{\hilbert_{3}}
\newcommand{\hilimo}{\hilbert_{i-1}}
\newcommand{\hili}{\hilbert_{i}}
\newcommand{\hilipo}{\hilbert_{i+1}}
\newcommand{\hillmo}{\hilbert_{\ell-1}}
\newcommand{\hill}{\hilbert_{\ell}}
\newcommand{\hillpo}{\hilbert_{\ell+1}}

% norms
\newcommand{\norm}[1]{|#1|}
\newcommand{\Norm}[1]{\left|#1\right|}
\newcommand{\bnorm}[1]{\big|#1\big|}
\newcommand{\Bnorm}[1]{\Big|#1\Big|}

\newcommand{\normx}[1]{\norm{#1}_{\X}}
\newcommand{\normy}[1]{\norm{#1}_{\Y}}
\newcommand{\normbanacho}[1]{\norm{#1}_{\banacho}}
\newcommand{\normbanacht}[1]{\norm{#1}_{\banacht}}
\newcommand{\normlt}[1]{\norm{#1}_{\lt}}
\newcommand{\normltrN}[1]{\norm{#1}_{\ltrN}}
\newcommand{\normltom}[1]{\norm{#1}_{\ltom}}
\newcommand{\normltoms}[1]{\norm{#1}_{\ltoms}}
\newcommand{\normltepsom}[1]{\norm{#1}_{\ltepsom}}
\newcommand{\normltmuom}[1]{\norm{#1}_{\ltmuom}}
\newcommand{\normltmorN}[1]{\norm{#1}_{\ltmorN}}
\newcommand{\normltmoom}[1]{\norm{#1}_{\ltmoom}}
\newcommand{\normhmoom}[1]{\norm{#1}_{\hmoom}}

% scalar products
\newcommand{\scp}[2]{\langle#1,#2\rangle}
\newcommand{\Scp}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\bscp}[2]{\big\langle#1,#2\big\rangle}
\newcommand{\Bscp}[2]{\Big\langle#1,#2\Big\rangle}
\newcommand{\sscp}[2]{\langle\!\langle#1,#2\rangle\!\rangle}

\newcommand{\scplt}[2]{\scp{#1}{#2}_{\lt}}
\newcommand{\scpom}[2]{\scp{#1}{#2}_{\om}}
\newcommand{\scpltom}[2]{\scp{#1}{#2}_{\ltom}}
\newcommand{\scpltoms}[2]{\scp{#1}{#2}_{\ltoms}}
\newcommand{\scphmoom}[2]{\scp{#1}{#2}_{\hmoom}}

% vectors and matrices
\newcommand{\btwovec}[2]{\begin{bmatrix}#1\\#2\end{bmatrix}}
\newcommand{\bthreevec}[3]{\begin{bmatrix}#1\\#2\\#3\end{bmatrix}}
\newcommand{\btwomat}[4]{\begin{bmatrix}#1&#2\\#3&#4\end{bmatrix}}
\newcommand{\bthreemat}[9]{\begin{bmatrix}#1&#2&#3\\#4&#5&#6\\#7&#8&#9\end{bmatrix}}

% preprint series UDE Mathematik
\newcommand{\preprintudemath}[5]{
\thispagestyle{empty}
\Large
\begin{center}SCHRIFTENREIHE DER FAKULT\"AT F\"UR MATHEMATIK\end{center}
\vspace*{5mm}
\begin{center}#1\end{center}
\vspace*{5mm}
\begin{center}by\end{center}
\begin{center}#2\end{center}
\vspace*{5mm}
\begin{center}#3\hspace{80mm}#4\end{center}
\newpage
\thispagestyle{empty}
\vspace*{210mm}
Received: #5
\newpage
\addtocounter{page}{-2}
\normalsize}

